Neural Cross-Lingual Coreference Resolution and its Application to Entity Linking

We propose an entity-centric neural cross-lingual coreference model that builds on multi-lingual embeddings and language-independent features. We perform both intrinsic and extrinsic evaluations of our model. In the intrinsic evaluation, we show that our model, when trained on English and tested on Chinese and Spanish, achieves competitive results to the models trained directly on Chinese and Spanish respectively. In the extrinsic evaluation, we show that our English model helps achieve superior entity linking accuracy on Chinese and Spanish test sets than the top 2015 TAC system without using any annotated data from Chinese or Spanish.

==> linking-short.tex <==
\section{Entity Linking model}
Most EL systems \citep{2007-emnlp-conll-cucerzan-wikipedia-NE-disambig,2011-acl-illinois-wikifier,globerson2016collective,yamada2016joint} do not  perform cross-lingual evaluations. Hence, we re-implement our recently proposed EL model by \citet{sil2018aaai} (henceforth, \sil) which is the current state-of-the-art (henceforth, ``SOTA'') for \textit{both} mono and cross-lingual EL. Given entities in a document, the model calculates sophisticated measures of similarity between the context of an entity in the document and the context of the candidate link's Wikipedia page which are fed into a feed-forward neural network. For details, we direct the reader to their paper. 

The coreference system clusters the mentions in a document into entities and subsequently, the EL system disambiguates them to Wikipedia. %based on the canonical mention of each entity. In this case, the canonical mention is the longest of all mentions belonging to an entity in a document.


% Most models proposed in the EL literature do not perform cross-lingual evaluations \citep{2011-emnlp-NE-disambig-yago,emnlp-chengroth-2013,2011-acl-illinois-wikifier,2006-eacl-bunescu-wikipedia-ne-disambig,2007-cikm-mihalcea-wikify,2007-emnlp-conll-cucerzan-wikipedia-NE-disambig,2008-cikm-milne-witten-wikifier,2009-kdd-wiki-ne-disambig-collective,globerson2016collective,lazic2015plato,yamada2016joint,ganea2016probabilistic}. So, we implement the recently proposed EL model by \citet{sil2018aaai} (henceforth, \sil) which is the current state-of-the-art (henceforth, ``SOTA'') for mono and cross-lingual EL. Given a query mention in a document, the model calculates several measures of similarity of the context of the mention in the query document and the context of the candidate link's Wikipedia page which are fed to a feed-forward neural layer with a \textit{sigmoid} non-linearity and then a softmax layer. For details, we direct the reader to their paper. 

% The coreference system first clusters mentions in a document into entities and subsequently, the EL system disambiguates the entities to their Wikipedia pages based on the canonical mention of each entity. In this case, the canonical mention is the longest of all mentions belonging to an entity in a document.
